Almanac: An API for Recommending Text Annotations For Time-Series Charts Using News Headlines

Authors often add text annotations to charts to provide additional context for visually prominent features such as peaks, valleys, and trends. However, writing annotations that provide contextual information, such as descriptions of temporal events, often requires considerable manual effort. To address this problem, we introduce Almanac, a JavaScript API that recommends annotations sourced from the New York Times Archive of news headlines. Almanac consists of two independent parts: (1) a prominence feature detector and (2) a contextual annotation recommender. We demonstrate the utility of the API using D3.js and Vega-Lite to annotate a variety of time-series charts covering many different data domains. Preliminary user feedback shows that Almanac is useful to support the authoring of charts with more descriptive annotations.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> figures/dataFlowDiagram.tex <==
\begin{figure}[t]
\centering
\caption{Data Flow}
\label{fig:dataFlowDiagram}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzstyle{box}=[draw, fill=blue!20, text width=5em, 
    text centered, minimum height=2.5em]
\def\blockdist{2.3}
\def\edgedist{2.5}

\resizebox{0.5\textwidth}{!}{% 
\begin{tikzpicture}
\node (data) [box] {Data Source};
\node (fDetect) [box,below right=4.5em of data, text width=6em]{Time Feature Detection};
\node (fAnnot) [box, right=5.5em of fDetect, text width=6em] {Time Feature Annotation};
\node (vis)  [box, above=of fDetect] {Visualizer \\ (Vega / D3)};

\path (data.south |- fDetect.west)+(0,-0.1) node (da) {};
\path (fAnnot.north |- vis.east)+(+0,0.1) node (fa) {};

\path [draw, ->] (data.south) to (da.north) to node[above] {Data} (fDetect.west) ;
\path [draw, ->] (data.east) to node[above] {Data} (vis.west |- data);
\path [draw, ->] (fDetect) to node[above] {Features} (fAnnot.west |- fDetect);
\path [draw, ->] (fAnnot.north) to (fa.south) to node[above] {Annotations} (vis.east);

\path (fDetect.east |- fAnnot.west)+(+0.5,0.25) node (t) {};
\node (toolbox) [below=3em of t,] {Annotation Tool};

\path (vis.north |- vis.west)+(0,0.25) node (f) {};
\node (frontend) [above=1em of f,] {Frontend};

\begin{pgfonlayer}{background}

% Draw Toolbox Box
\path (fDetect.west |- fAnnot.north)+(-0.5,0.25) node (ta) {};
\path (toolbox.south -| fAnnot.east)+(+0.25,-0.25) node (tb) {};
\path[fill=yellow!20,rounded corners, draw=black!50, dashed]
            (ta) rectangle (tb);

% Draw Frontend Box
\path (vis.west |- frontend.north)+(-0.25,0.25) node (fa) {};
\path (fDetect.south -| fDetect.east)+(0.25,-0.25) node (fb) {};
\path[fill=red!20,rounded corners, draw=black!50, dashed]
            (fa) rectangle (fb);
            
\end{pgfonlayer}

\end{tikzpicture}
}%
\end{figure}


==> figures/dataFlowDiagramV2.tex <==
\begin{figure}[t]
 \centering
    \includegraphics[width=\linewidth]{figures/dataflow.pdf}
    \vspace{-2em}
    \caption{The two main components of the \toolname{} API are a feature detector (blue) responsible for identifying visually prominent chart features and an annotation recommender (green) responsible for ranking headlines from an annotation database with respect to contextual relevance. \maneesh{Perhaps remove this figure}}
    \vspace{-1em}
    \label{fig:dataFlowDiagram}
\end{figure}

==> figures/persistence_src.tex <==
 \begin{figure}[b]
  \centering
     \includegraphics[width=\linewidth]{figures/persistence.pdf}
     \vspace{-2em}
     \caption{\toolname's chart feature detector computes the prominence of peaks in this stock price chart, as their persistence lifetimes (length of red lines). The longest lifetimes are most persistent and therefore ranked most prominent. Here we see the top six peaks and their lifetimes. \maneesh{Perhaps remove this figure.}}
     \vspace{-1em}   
     \label{fig:persistence}
 \end{figure}



==> figures/usingAPI_src.tex <==
\begin{figure*}[t!]
 %\centering
    \includegraphics[width=\linewidth]{figures/usingAPI.pdf}
    \vspace{-2em}
    \caption{Chart authors use the \toolname{} API in two steps. Given a time-series chart (left) of stock price data for Tesla Inc.~\cite{AlphaVantage2022Stock}, the author applies the {\ttfamily getChartFeatures} command to return the most prominent peaks and valleys in the chart (left, marked in red). Authors can manually mark point and trend features as well. The author then selects the most prominent peak and runs \toolname's {\ttfamily getAnnotations} command to obtain a  set of contextual headlines (middle top). By default, the highest-ranked headline is chosen as the annotation, but the author can manually examine the other headlines to see if a better headline is available. The author uses the top-ranked default headlines to create the final chart (right).}
    \vspace{-1em}   
    \label{fig:usingAPI}
\end{figure*}




==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/05_evaluation.tex <==


We conducted a web survey to assess whether \toolname's annotation recommender suggests relevant annotations for the prominent features in time-series charts. 
%\subsection{Participants}

\vspace{0.5em}
\noindent
{\textbf \em Method.}
The survey consisted of seven questions. Each question displayed a time-series chart from a dataset (e.g., COVID-19 cases, Mass Shooting Deaths, U.S. President Approval Rate, Euro 1-yr Swap Rate) with one visual feature marked with a red dot. Three annotations were chosen from the ranked set of headlines generated by the annotation recommender - the top-ranked headline, the bottom-ranked headline, and one picked from the middle of the distribution of scores. 
The headlines were displayed in random order below the chart. 
The instructions to the participants were as follows:

``Above is a graph of the \textsc{<chart title>}, with a visually salient peak at \textsc{<date>} marked with a red dot. 
Below is a set of New York Times headlines that could be used to annotate the peak. For each headline, mark it as providing \textit{Useful Context} for understanding the peak, or \textit{Not Useful}, by dragging it to the appropriate box.
For the Useful Context box, rank the headlines by dragging them up and down, with 1 as the Most Useful and 3 as the Least Useful. Note: You should click on each headline to see the lead sentence of the New York Times article before deciding on its usefulness.''

We provided a free-form response field at the end of each question, prompting the participant to describe their justification for their preferences. The survey instructions and data are included in the supplementary material.

We recruited 10 participants through a company mailing list and social media channels. All participants were required to be fluent in English and complete the survey on a desktop or laptop device.


\vspace{0.5em}
\noindent
{\textbf \em Survey results.}
Overall, we found that \toolname's top-ranked headlines were marked as {\em useful} by 95.7\% of participants. This was followed by the middle-ranked headline at 31.4\% and the bottom-ranked headline at 20\% as being useful. 
%
In terms of the ranking preferences of the headlines that participants indicated as useful, \toolname's top-ranked headline was ranked as most useful 85.7\% of the time, followed by the middle-ranked headline at 7.1\%, and the bottom-ranked one at just 2.9\%.

Participants' free-form feedback supported these results. For the chart showing the death from mass shootings, $P4$ commented that the top-ranked annotation, \textit{``Police Yet to Determine Motive in Virginia Tech Shooting''} was \textit{``the only headline that seems to reference a mass shooting.''} and $P1$ said \textit{``the 1st ranked one is more about the whole situation (mentions all 32 victims) so it is more useful, the 2nd ranked one is about 1 person when the graph is about overall numbers so it is less relevant.''} Participants also appreciated that the top-ranked headline, `\textit{`More countries shift to self-administered antigen tests in a race to stop Omicron''} in the COVID-19 cases chart contained detail about the event. $P5$ commented, \textit{``The `Omicron' headline is the only useful headline as it implies that Omicron is running rampant and provides context on how countries are responding, which could provide context for future data points.''} Finally, a few participants found both the top- and middle-ranked headlines to be relevant to the highlighted feature in the chart. $P4$ remarked, \textit{``The two useful headlines refer to the Euro flailing or in crisis, both descriptions of the trend of the chart.''}


\vspace{0.5em}
\noindent
%{\bf \em Discussion.}\vidya{calling this a discussion, feels sparse.}
Together these survey and feedback results suggest that \toolname{} is able to effectively recommend headline annotations that provide useful context to readers across a variety of different time-series data sets. 



==> sections/06_futurework.tex <==
% While \toolname{} provides a simple API for annotating time-series charts with NYT headlines, it does have some limitations that can inspire future work.
% %\maneesh{Maybe kill this section for the short paper. Or significantly shorten.}

% % \vspace{0.5em}
% % \noindent
% % {\bf \em Extending the headline corpus.}
% The built-in NYT corpus covers news headlines and may not include certain types of less newsworthy temporal events; nor does it cover events that happen at very long (years) or very fine (seconds) timescales. Most headlines in our corpus are about events that are days to months long. Future work should consider incorporating other annotation sources such as Google search results, Wikipedia Events~\cite{Wikipedia2022Events}, or even domain-specific corpora as part of the annotation recommender. %\maneesh{I think we have done this. I would remove it from here.}


% \vspace{0.5em}
% \noindent
% {\bf \em Time alignment of the headlines to the data.}
% \maneesh{I would probably remove this one.}
% \toolname{} considers the published date of the NYT articles to align with the events occurring in the chart. However, because NYT news articles are sometimes published days (or in the case of historical analysis weeks and months) after the event, the headlines may be temporally offset from the actual event. 
% Future work could analyze the annotation database as a preprocess to better align articles with events relevant to the data. Alternatively, it may be possible to  
% provide an API-level control, that would allow chart authors to offset the alignment between the annotation database and the data in the chart. \maneesh{Can we give example of this one.}

%As with any corpus-based approach, our API does have some limitations. The NYT corpus is primarily news headlines that cover a limited set of temporal events. The Contextual Annotation Recommender considers the published date of the NYT articles to align with the events occurring in the chart. These annotations are sometimes offset temporally from the actual events \vidya{example?}. Future work should consider incorporating other corpora like Google search results, Wikipedia Events~\cite{}, or even domain-specific corpora as part of the Contextual Annotation Recommender API command. 

%\vspace{0.5em}
%\noindent
%{\bf \em Other approaches to rank relevant annotations.}
%\toolname's annotation recommeder ranks relevant articles based on the time range of the prominent feature and a TD-IDF term weighting approach. Other directions worth investigating include considering term proximity approaches~\cite{Rasolofo2003TermPS} that rank documents with query terms in close proximity as more relevant than articles with terms scattered throughout the text of the article. \maneesh{I don't follow what close proximity means here. Not sure why this is worth pursuing. If it would be a better approach why didn't we use it. I might cut this one. }

% \vspace{0.75em}
% \noindent

 
%other applications where these two API commands could be used, including:
%\maneesh{I'd probably remove most of the future work. here} 
% \vspace{0.5em}
% \noindent 
%{\bf \em Feature-based simplification.} 
% Recent work has explored the problem of rendering charts at different sizes while preserving their prominent features~\cite{semanticresizing:2021}. \toolname's prominence feature detector command could be used in automating the simplification process for responsive chart design and for different target displays.

% Talk about generalization
% Recent research has explored how readers integrate information from text and charts together when they take away information~\cite{Kim2021,stokes:2022}. \toolname's prominence feature detector command could be used in tools to help authors check if prominent features in charts are in agreement with the captions they include. 
% Similarly, future applications could explore novel visual analytics tools to suggest better captions or alternative chart representations so that prominent features in charts and text describing them, are in agreement.  \maneesh{I'm a little concerned about this one.}\vidya{we can nuke this portion for various reasons}
%Our current API simply renders the annotations adjacent to the prominent features in the chart. %Future work could explore layout algorithms for both formatting and rendering annotations on charts to minimize visual clutter and for better readability.

% \vspace{0.5em}
% \noindent 
% {\bf \em Article recommendations.}
% \toolname's annotation recommender not only identifies relevant headlines, it also scores those headlines and the terms within them using our time-based variant of TF-IDF. This metadata about the headlines could be useful to find additional articles (e.g., from sources beyond the NYT) that are related to the event topic and thereby support the creation of data narratives that go beyond annotation recommendations. 

% \vspace{0.5em}
% \noindent 
% {\bf \em Search interfaces.} The text metadata describing prominent features in charts could also be used as part of search interfaces commonly found in platforms like Tableau Public~\cite{tableaupublic} and document search engines such as Google, to find pre-authored charts based on the input search terms. The terms and weights describing these prominent features can be used for Search Engine Optimization (SEO) to boost relevant charts based on the search queries. In addition, SEO could improve visibility by not only finding charts in these search interfaces but also surfacing other relevant documents that describe and provide additional context to the events.


% There are other uses for these two API commands
% \maneesh{Talk about other uses of API in discussion -- e.g. peak detector could be used to highlight prominent parts of the chart even without annotation, article recommendations could be used scrape additional charts from news articles, or some such.} 
% Getting features can be useful for highlighting them

% Similarly, getting related articles, recommend additional articles, find related charts: search metadata. SEO

% Beyond visualization: SEO in the context of articles and charts




